Kinematic Modeling of Handed Shearing Auxetics via Piecewise Constant Curvature

Handed Shearing Auxetics (HSA) are a promising technique for making motor-driven, soft, continuum robots. Many potential applications from inspection tasks to solar tracking require accurate kinematic models to predict the position and orientation of these structures. Currently there are no models for HSA based continuum platforms. To address this gap we propose to adapt Piecewise Constant Curvature (PCC) Models using a length change coupling matrix. This models the interaction of HSA structures in a 2x2 array. The coupling matrix maps the change in motor angles to length changes and defines the configuration space in our modified PCC Model. We evaluate our model on a composite movement encompassing bending, extension and compression behavior. Our model achieves a positional accuracy with mean error of 5.5mm or 4.5% body length and standard deviation of 1.72mm. Further, we achieve an angular accuracy with mean error of -2.8$^\circ$ and standard deviation of 1.9$^\circ$.

==> 3NeuralNet.tex <==
\section{Neural Network Model}
% .5-1 pages

A single layer, feed forward network was created in MATLAB for non-linear regression as a point of comparison against the derived ECC model. The inputs to the network were the four $\theta$ variables used to actuate the HSAs and the outputs were the position of the platform's center $\bm x$ in $x, y, z$ and the imaginary parts $q_x, q_y, q_z$ of the platform's quaternion $\bm q$. The real part of the quaternion $q_w$ was not part of the output because the quaternion $\bm q$ is unit length and thus only three parts are needed to determine the fourth. The network was trained using mean square error (MSE) as the cost function and the Levenberg-Marquardt backpropagation algorithm. The 2401 theta state samples were randomly divided into training and validation sets at a 7:3 ratio. Training time for all networks were less than 1 minute on a machine with an Intel\textsuperscript{\textregistered} Core\textsuperscript{\texttrademark} i-7 and 32 GB of RAM.

Fig.~\ref{fig:NN_performance} shows the MSE plot for a network with a single hidden layer with 20 neurons and a table showing final performance of networks with various hidden layer sizes. The MSE in this training is the raw error associated with position and quaternion values. Table~\ref{tab:NN_compare} shows that the error on the validation dataset does continue to decrease with increased hidden layer size; however, this also results in an overfitting of the data, where the training error continues to decrease while the validation performance only improves marginally. The network with 20 neurons was used as the final comparison point with the ECC model because it was heuristically determined to have the best performance overall in terms of validation and test error although it should be noted that the network with only 5 neurons also performed nearly as well in terms of absolute error. 

\begin{figure}[h]
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.8\linewidth]{Media/mse_epoch_20neurons.png}    
        \label{fig:NN_mse}
        % \caption{\todo{CAPTION}}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Single layer 20 neuron training performance over time.}
    \label{fig:NN_performance}
    \vspace{-4mm}
\end{figure}

\begin{table}
    \centering
    \begin{tabularx}{.9\linewidth}{| X | X | X | X |}
        \hline
        No. \newline Neurons & No. Free Parameters & Training MSE & Validation MSE \\
        \hline
        5           & 61                           & 4.38E-5      & 4.47E-5       \\
        20          & 226                           & 7.35E-6      & 8.95E-6       \\
        50          & 556                          & 4.37E-6      & 5.77E-6       \\
        100         & 1106                           & 3.86E-6      & 6.28E-6       \\ 
        \hline
    \end{tabularx}
    \caption{Comparison of different network sizes.}
    \label{tab:NN_compare}
\end{table}


==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/0Introduction.tex <==
\section{Introduction}
% .5-1 pages

%\todo {
%\begin{itemize}
%    \item uses of move and point actuators 
%    \item the importance of compliant robotics (resilience)
%    \item how HSAs can be better than fluid based
%    \item current exploration of HSA space is mechanical characterization but not controls
%    \item exploration of controls in soft robotics
%    \item alt techniques to PCC models
%    \item PCC modeling limitations
%\end{itemize}}

The ability to orient robotic arms in space is critical to a wide range of applications. In inspection tools the ability to point cameras and other sensors ensure our critical infrastructure is well maintained and objects we purchase are fabricated properly. Satellite communication systems require accurate angular tracking to ensure connections are not lost~\cite{sattelite5342320}\cite{innovationsSatelliteCommunications}. In energy systems it enables sun tracking for solar panels and solar thermal systems\cite{MOUSAZADEH20091800}\cite{ROTH2004393}. All of these applications necessitate that they are resilient to contact with their environments which is a strength of soft robotics\cite{SoftRoboticsReviewhttps://doi.org/10.1002/adem.201700016} \cite{resulience10.3389/frobt.2017.00048} \cite{Rus2015}. An electrically driven soft robot able to accurately point would be of broad utility.

Current research on electrically driven soft actuators has shown that handed shearing auxetics (HSAs) have proven very promising \cite{Lipton632}. They are capable of linear expansion, and have distributed compliance like pneunets\cite{mosadegh2014pneumatic}, but are driven by motor torques rather than fluid flows.  Recent research has focused on applying HSAs to gripping tasks\cite{Chin20198794098,chin2020multiplexed}, sensorization\cite{chin2019simple,chin2019automated} and  mechanical characterization\cite{Truby2021-9326362}, but there have been no proposed control methods that describe the actuation of HSAs. 

We use a common design of two sets of opposite handed HSAs to form a 2x2 HSA platform\cite{Lipton632} as seen in Fig.\ref{fig:hero}. 
%This system has 4 degrees of freedom with four servo motor angles as inputs and the position of the top platform and its orientation as the output state.
Its  simple design makes it an ideal section for a soft robotic inspection arm, while its large platform area makes a single section ideal for used as a pointer for solar panels or communication equipment. Despite the simplicity and utility of the design, without a model it cannot be of use or properly controlled. 

We therefore look to adapt the existing soft robotics literature on control and apply them to HSA systems in order to enable electric soft robotic pointing systems and future multi-segment arms. We look to a common soft robot modeling method,  Piecewise Constant Curvature (PCC)\cite{Walker2006-1588999,Jones2010-doi:10.1177/0278364910368147}. PCC models assume that arms can be modeled as composites of rods that bend at a programmable radius and length that rotate relative to each other. Typically this bending is induced by differential pressure on chambers\cite{katzschmann2019dynamic}. Because HSAs are extensible and compliant, we needed to develop a constant curvature model that captures this behavior. Extensible PCC models capture the arc length changes of the segments as they are actuated. 




%hero figure
\begin{figure}[t]
    \centering
    \hfill
    \centering
    \includegraphics[width=1\linewidth]{Media/FinalHero.png}
    \captionsetup{justification=centering}
    \caption{Modeling a 2x2 HSA platform with Extended Piecewise Constant Curvature}
    \label{fig:hero}
    \hfill
    \vspace{-0.75cm}
\end{figure}

Our work maps the actuation space to segment lengths and accounts for inter-segment coupling with 5 parameters in a coupling matrix. We demonstrate that the PCC is more predictive than simple kinematic models with and without coupling. We evaluate this model on a  composite movement to combine bending, extension and compression of the HSAs. Our proposed model achieves a positional accuracy with mean error of 5.5mm or 4.5\% body length and standard deviation of 1.72mm. For the orientation, we achieve an angular accuracy with mean error of  -2.8$^\circ$ and standard deviation of 1.9$^\circ$.

In this paper we:
\begin{itemize}
    \item Model the interactions between individual HSAs on a platform.
    \item Adapt the Piecewise Constant Curvature model to a HSA driven platform with 4 lengths.
    \item Validate the modified PCC model through experiments on a HSA platform.
\end{itemize}


==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/1Background.tex <==
\section{Background and Related Work}
% .5-1 pages


%\begin{itemize}
%    \item HSAs
%    \item Modeling of soft Robotics
%    \item PCC Model %Aman
%\end{itemize}}


%The defining characteristic of auxetic materials is the presence of a negative poisson's ratio. Unlike most materials under tensile loading, these materials expand as a result of their periodic links and joints structure \cite{Lipton632}. These periodic patterns can fill 3D space , or in the case of HSA actuators in this work, tile 2D surfaces like the lateral surface area of a cylinder. Driven by the angle $\theta$ between two links, each unit cell expands or contracts as a result of loading, collectively deforming structure they create. The HSAs in this work, which couple global shearing from twisting to expansion along the axis of rotation, are known as shearing auxetic cylinders \cite{Chin20188404904}. Auxetic metamaterials normally have a symmetric point in their trajectory, enabling them to transition from one handedness to another. This symmetry is purposely broken in HSAs, resulting in a single chiral shear motion. In order to create a HSA of opposite handedness, a simple reflection of the periodic pattern is sufficient \cite{Truby2021-9326362}.

%While traditional fluid based soft robots have been demonstrated as very capable at some inspection style tasks like archaeological exploration and search and rescue operations\cite{akamura8917931}. Electrically driven soft robots would have an advantage in independently pointing large arrays or integrating with existing infrastructure. Most fluid based soft actuators require bulky and often rigid systems to generate the pressure differentials they use to actuate. Add on the additional need for electronic controls and the block diagram for such a system becomes complicated very quickly. With electrically driven soft actuators, there is no need for additional energy conversion which improves efficiency and robustness since there are fewer systems that can fail \cite{fluidconversionlossesdoi:10.1089/soro.2014.0018} \cite{Chin20188404904}.

Soft robots have been usually driven by variable length tendons and pneumatic actuation and more recently, electroactive polymers \cite{Shintakeelectroactive}.Handed shearing auxetics (HSAs) are a new category of material that enables electric soft robots. HSAs couple auxetic expansion with shear as a result of their periodic links and joints structure \cite{Lipton632}. Auxetic metamaterials normally have a symmetric point in their trajectory, enabling them to transition from one handedness to another. This symmetry is purposely broken in HSAs, resulting in a single chiral shear motion. In order to create a HSA of opposite handedness, a simple reflection of the periodic pattern is sufficient~\cite{Truby2021-9326362}. When tiled on a cylinder, the HSA patterns couple global shearing from twisting to expansion along the axis of rotation~\cite{Chin20188404904}. These structures are compliant by nature, allowing for spring like responses to impacts or other disturbances. Their responsiveness to twisting allows for them to form linear compliant actuators driven directly by motor torques when placed in pairs~\cite{Lipton632}. Most applications of HSAs have been in grippers, since they require no model to be able to grasp successfully~\cite{Chin20198794098,chin2020multiplexed,chin2019simple,chin2019automated}. 

%\todo{paragraph on PCC modeling in soft robots.}
Modelling the motion of soft robots is challenging due to their inherent infinite degrees of freedom.Various research works have shown that finite element methods and other numerical techniques can be used to describe the behaviour{\cite{zhang2016kinematic}}{\cite{elsayed2014finite}}. But their inability to provide a closed form solution limits their adoption. An alternate approach - piecewise constant curvature models have been found to be more effective in defining the behaviour, where the robotic structure is broken into continuous segments with constant curvatures providing an easy way to model a system which is differentiable everywhere{\cite{8722799}}{\cite{webster2010design}}. PCC modelling includes two mappings - 1) From actuator space to the configuration space ($s$,$\kappa$,$\phi$) which describes the curvature produced by the continuum robot and 2) from configuration space to pose which defines the position and orientation of the end-effector. 

The first mapping is unique to the type of robotic system such as pneumatic or tendon actuated arms{\cite{renda2014dynamic}}{\cite{talas2020design}}. The second mapping is a standard kinematic transformation from the arc parameters to the coordinate system of the task space. This transformation can be achieved through different conventions and definitions{\cite{Walker2003-https://doi.org/10.1002/rob.10070}}. One of those techniques uses the modified Denavit-Hartenberg (D-H) approach to define a transformation matrix that maps the configuration space to the task space.In this modified D-H method, the continuum robot is defined as a virtual rigid-link robot allowing for convenient closed form calculations \cite{Walker2006-1588999}.    

On first glance, one might be inclined to use a parallel manipulator model for the kinematics of HSA based robotic section, since both HSAs and Stewart platforms rely on a change of length\cite{dasgupta2000stewart}. However, unlike links in a Stewart platform HSAs are always perpendicular to their base. This is most similar to traditional pneunet based structures which have been modeled using PCC \cite{della2020data}. %Since future applications may rely on compounding multiple HSA sections, a PCC model would provide the added advantage of generating a centerline for predicting contact. 

%Aman
%\todo{Explain and compare why pcc vs parallel manipulator approach}



%A significant amount of progress has been made in modelling the behaviour of soft robots as continuum robots. One of those approaches approximates the robotic arm as a series of constant curvature arcs \cite{webster2010design,walker2020soft}.  
%We expand the model presented by Walker~, for four extensible actuators by mapping their lengths to curvature defining parameters $s, \kappa, \phi$ and $\psi$ of a virtual link of the center of the top platform. $s$ represents the arc-length of the centerline, $\kappa$ represents the curvature of the line, $\phi$ represents the rotation of the line around the base, and $\psi$ represents the rotation of the centerline around itself.  

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics{ConfigDrawing.pdf}
        \caption{Configuration parameters for the PCC model}
        \label{fig:configuration}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{Media/rest_state.png}
        \caption{Assembly at rest.}
        \label{fig:rest_position}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.21\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{Media/actuated_position.png}
        \caption{Assembly after actuation.}
        \label{fig:actuated_position}
    \end{subfigure}
    \hfill
    \caption{The piecewise constant curvature model maps the location of a robot section using curvature($\kappa$) arclength ($S$) and }
    \label{fig:configurationFull}
\end{figure}


==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/2A-Hardware.tex <==
\section{HSA model and Platform Design}
\label{sec:HSADesign}
HSAs, though not conventional linear actuators, do extend when the connected motor is activated, so the extension of a single HSA is a function of the motor's angle of rotation $\theta$. We made our HSAs on a Carbon M1 out of FPU50 with a inner diameter of 22.98 mm and thickness of 2 mm. 
To establish mapping between angles and HSA length we conducted a force vs. displacement test using an Instron Universal Testing Machine at step angles of 30\textsuperscript{o} from 0\textsuperscript{o} to 180\textsuperscript{o}. At each step we observed the length at which the force was zero. We observed that the extension is approximately linearly dependent on the angle and as a result the length of an actuator can be modeled as linear function of the angle of the servo motor.  We found an equation of the form $L = \alpha_{0}\ast \theta   + \alpha_{1}$ with $\alpha_{0}=$ 0.124, $\alpha_{1}=$ 0.119 fit the data with an $R^2=$ 0.99. 

%\begin{figure}[h]
%    \centering
%    
%    \begin{subfigure}[c]{0.4\linewidth}
%    \centering
%        % \begin{frame}{ 
%        \includegraphics[width=\linewidth]{Media/NSANaiveA%rial.png}%}    
%        % \end{frame}
%    \end{subfigure}
%    % \hfill
%    \begin{subfigure}[c]{0.5\linewidth}
%    \centering
%        \includegraphics[width=\linewidth]{Media/uncoupled%_theta_mapping.png}
%    \end{subfigure}
%    
%    \captionsetup{justification=centering}
%    \caption{Finding the rest lengths of a left-handed HSA %for a given rotation $\theta$.\tk{Need angles legent for %B, Need labeling A and B}}  
%    \label{fig:HSAnaive}
%\end{figure}

\subsection{The 2x2 Platform}
% 1-1.5 pages

\begin{figure}[htbp]
    \centering
    \begin{frame}{ 
    \includegraphics[width=.7\linewidth]{Media/HSAPlatformLabeledArial.png}}    
    \end{frame}
    \captionsetup{justification=centering}
    \caption{The 2x2 HSA test platform. The top figure indicates the handedness of each HSA in the platform.}
    \label{fig:HSA_Platform}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{workspace.pdf}
    \captionsetup{justification=centering}
    \caption{Workspace of the HSA platform }
    \label{fig:workspace}
\end{figure}

A 2x2 HSA platform Fig.~\ref{fig:HSA_Platform} was designed, 3D printed, and assembled. It has four independent HS-785HB servos in the base connected to to four vertical HSAs. The HSAs are attached together to a ridged platform on top. The servos are controlled via a Pololu Mini Maestro 12-Channel USB servo controller and are powered with 6V and the system draws up to 3 watts during testing. The servos are mounted to the base in an angled pattern at 42$^{\circ}$. This arrangement allows for a 43.68 mm center to center distance between HSAs. A key feature of the actuator assembly is the presence of opposite handed HSAs. In order to balance the net torque on the top platform produced from the independent rotation of each HSA, each handed pair of actuators are arranged diagonally in the 2x2 grid as shown in the top right corner of Fig.\ref{fig:HSA_Platform}. Thus, two of the servos rotate clockwise and two rotate counterclockwise to extend each HSA. Therefore there is no need for a strain constraint layer or a solid core in the structure. This allows the platform to change in length and extend in the Z direction in addition to bending. The resulting workspace of a single structure can be seen in Fig~\ref{fig:workspace}. 

%The adaptors have four slots in which small nuts can be inserted. After the HSA is placed onto the mount, the four radial holes printed in the HSA align with through holes in the adaptor and connect to the inserted nuts. This fastener arrangement is also used in the top platform design, which connects all four HSA together in their neutral, rest length state. 
%The top platform is designed to provide a sufficiently ridged structure, while minimizing unnecessary mass at just 30.75 grams.
%During testing at 30$^{\circ}$ increments up to 180$^{\circ}$ rotation at the base of each HSA, the actuators are capable of lifting the platform vertically up to 31 mm above the resting position. 

% \begin{figure}[htbp]
%     \centering
%     \begin{frame}{ 
%     \includegraphics[width=.7\linewidth]{Media/HSAExtensionArrow.png}}    
%     \end{frame}
%     \captionsetup{justification=centering}
%     \caption{Extension of all four HSAs to $180^\circ$}
%     \label{fig:HSA extension}
%     \vspace{-4mm}
% \end{figure}

%The Flex 13 boasts 30-120 FPS frame rates, 1.3 Megapixel resolution and sub-millimeter marker precision on the order of 100 microns in most applications.
%Paragraph on following carbon's printing guidelines. Either here or error subsection in results
%Pololu's software allows for customization of the speed and acceleration of all servos independently, and allows pulse width modulation (PWM) target values to be input and combined into sequences with the desired delay between movements.

%To ensure even loading of the HSAs, we randomly chose the next state for the system and ensured the platform was sent back to rest between each move. 
%

 







==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/2ModelingPCC.tex <==
\section{Kinematic Models}

% \todo{
%   \item discuss error and range for linear model and why it failed
%   \item compared to straight mixing model (beta  matrix)
% }
%For our models to be useful we need to determine the position of the center of the top platform and its orientation from the controlling the angles of rotation of individual actuators in the system.  We model our chosen 2x2 HSA platform as extensible curvature model as shown in Fig.~\ref{fig:hero} to compute the forward kinematics of the system. This is made possible because the actuators subtend arcs when they are subjected to uniformly applied tension on one end and constraint loading on the other, leading to expansion of 2D surfaces of the actuator. With the individual arc lengths and straight lengths of the actuators we can ascertain the orientation and position.
%


\subsection{Mapping $\theta$ to Length}

%The key parameter that drives a single HSA is the angle through which the motor rotates which we define here as $\theta$. An increase in rotation extends the HSA provided it is constrained on the other end. To build this relationship we use an Instrob n Universal Testing Machine which demonstrated a linear mapping between length of the actuator vs. $\theta$.%
In the 2x2 HSA platform, all the actuators are fixed in position at the base and         coupled together with the top platform acting as a second common link between them. If HSA actuators were rigid length change actuators, the system would appear to be over constrained since only 3 heights relative to one plane are needed to define another. HSAs however are compliant, with the ability to compress and extend in response to external forces in addition to twist driven length changes. This means that the length of any of the actuators at any time is dependent on length of other actuators (and by extension their theta states). We use our previous observation to model the length of actuators as linearly dependent on theta values of all actuators. If $\vec{L}$ represents the lengths of the actuators then we can write $\vec{L}$ as
\begin{equation*}
    \vec{L} = \bar{\beta_0} \cdot \vec{\theta}   + \vec{\beta_{1}}.    
\end{equation*}

The $\beta_0$ matrix establishes the extent of coupling between the actuators and $\vec{\theta}$ and $\beta_1$ vector establishes their height at rest. Consequently, any change in the dimensions of HSA would affect the coupling. For this reason we determine $\beta_0$ and $\beta_1$ for our chosen design through regression modelling.
 
The $\beta_\text{0,regression}$ matrix does not result in a perfectly symmetric matrix. To enforce symmetry we break the $\beta_0$ matrix up into two components, $\beta_\text{0,symmetric}$ and $\beta_\text{0,deviation}$ such that $\beta_\text{0,symmetric}$ + $\beta_\text{0,deviation}$ = $\beta_\text{0,regression}$. The $\beta_\text{0,symmetric}$  matrix is then found by taking the mean of the diagonals, making a circulant matrix. We then use $\beta_\text{0,symmetric}$ as $\beta_0$. Further, we average out the terms in $\beta_1$ to build a measure of the height of the actuators at rest. 




\subsection{Piecewise Constant Curvature approximation of HSAs}


%The bending behavior of a single HSA, requires defining the curves produced by actuation. A na\"ive approach would be to model each HSA as coupled linear actuators from their base to their end and ignore the curvatures; however, this would only give positional and angular information of the platform. Our method fully describes the position of the whole system in space and thereby can be extended to include collision detection and dynamic modeling\cite{Rus2015}.

We choose the central point between all HSAs to be the distal end of our constant curvature rod as seen in Fig.~\ref{fig:actuated_position}. From there, we define the origin to be the point between the bottom of all the HSAs.
%Naturally a coordinate system that is tailored to defining these curves is ideal and the best one is the $s, \kappa, \phi$ system which can then be translated to the $x, y, z$ coordinate system when needed. An additional complication is that our system has four coupled HSAs to be modeled as unique curvatures, but we desire to know the curvature and location of the center of the system in space.
In order to model the HSA assembly we first establish the straight lines connecting the ends of the HSAs. Fig.~\ref{fig:rest_position} shows the HSA assembly represented as two square, rigid bodies of the same dimension $m$, with corners $P = \{A, B, C, D\}$ and $\bar{P}=\{\bar{A},\bar{B},\bar{C},\bar{D}\}$ called the ``platform'' and ``base'' respectively. We also initially constrain all points in $P$ to lie in the same plane $\mathcal{P}$ and all points in $\bar P$ to lie in the plane $\mathcal{B}$. The platform and base are separated by the set of rigid links with lengths $L=\{l_A, l_B, l_C, l_D\}$ where $l_J=\|\bar{J}J\|_2$ for $J \in P$ and have geometric centers. We note that due to this geometry the distance ${l_S}$ from the center of the platform to the origin i.e. the center of the base is given by: 
%$S$ and $\bar{S}$
% \begin{figure}[h]
%     \centering
%     \hfill
%     \begin{subfigure}[t]{0.15\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{Media/rest_state.png}
%         \caption{Assembly at rest.}
%         \label{fig:rest_position}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.21\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{Media/actuated_position.png}
%         \caption{Assembly after actuation.}
%         \label{fig:actuated_position}
%     \end{subfigure}
%     \hfill
%     \captionsetup{justification=centering}
%     \caption{ECC model of HSA assembly at rest and after actuation.}
%     \label{fig:ECC_model}
% \end{figure}

%Once actuated, we take a corner pair, e.g. $(A, D)$, and find a point $D'$ on $\bar{D} D$ such that $l_A = l_{D'}$ as shown in Fig.~\ref{fig:triangle}. We then also draw a point from $A$ to a point $D''$ such that $AD'' \perp \bar{D}D$ bisecting the triangle made by $AD'D$. The section $D'D$ is split by $D''$ with total length $2h_D$. We repeat this process from point $A$ to the other linkages forming a plane $AB''C''D''$  with additional distances $h_B, h_C, h_D$. From the perspective of corner $A$, $h_A$ is zero, but it should also be noted that the other $h_J$ values are allowed to be negative in the cases where corner $A$ is higher than the other corners.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=.45\textwidth]{Media/triangle.png}
%    \caption{Side view of assembly after actuation. Not to scale.}
%    \label{fig:triangle}
%\end{figure}

%Points $AB''C''D''$ form a new plane $\mathcal{H}$ where $h_B, h_C,$ and $h_D$ are the standoff distances between $\mathcal{H}$ and $\mathcal{P}$. We also define the stand off from center $S''$ to center $S$ as $h_S$ as shown in Fig.~\ref{fig:plane_h}. We use $h_S$ for deriving the distance of the center of the platform to the center of the base, which must be expressed in the known lengths $L$. We obtain Fig~\ref{fig:cut_section} by observing a cut section along the diagonal of the platform. Knowing that the triangles $ACC''$ and $ASS''$ are similar and that $AS''$ is half the distance to $AC''$, we can easily see that 

%\begin{equation} \label{eq:hs}
%    h_S = \frac{h_C}{2} =  \frac{l_C - l_A}{4}
%\end{equation}
%and



\begin{equation} \label{eq:ls}
    l_S = \frac{l_A + l_C}{2} = \frac{l_B + l_D}{2} 
\end{equation}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=.45\textwidth]{Media/plane_h.png}
%     \caption{Stand off distances between plane $\mathcal{H}$ and $\mathcal{P} $.}
%     \label{fig:plane_h}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \hfill
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{Media/top_platform.png} 
%         \caption{Head on view of platform.}
%         \label{fig:top_platform}  
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{Media/cut_section.png}
%         \caption{Cut view $V$.}
%         \label{fig:cut_section}
%     \end{subfigure}
%     \hfill
%     \label{fig:top_view}
    
%     \caption{Top of platform and standoff distances between $\mathcal{P}$ and $\mathcal{H}$.}
    
% \end{figure}

%\begin{figure}
%    \centering
%    \begin{subfigure}{.9\linewidth}
%        \includegraphics[width=1\textwidth]{Media/plane_h.png}
%        \caption{Stand off distances between planes $\mathcal{H}$ and %$\mathcal{P} $.}
%        \label{fig:plane_h}    
%    \end{subfigure}
%    % \hfill
%    \begin{subfigure}{0.45\linewidth}
%        \centering
%        \includegraphics[width=1\textwidth]{Media/top_platform.png} 
%        \caption{Head on view of platform.}
%        \label{fig:top_platform}  
%    \end{subfigure}
%    % \hfill
%    \begin{subfigure}{0.45\linewidth}
%        \centering
%        \includegraphics[width=1\textwidth]{Media/cut_section.png}
%        \caption{Cut view along $AC$.}
%        \label{fig:cut_section}
%    \end{subfigure}
%    % \hfill
%    \label{fig:top_view}
%    \caption{Determining $h_S$ from planes $\mathcal{P}$ and %$\mathcal{H}.$}
%\end{figure}


%Ultimately we wish to derive $\kappa$ which is the curvature of the arc segment from point $\bar{S}$ to $S$ as shown in Fig.~\ref{fig:actuated_position}. In order to derive the full $\kappa$ we first derive the curvatures for each of the individual linkages
%$\{\kappa_A, \kappa_B, \kappa_C, \kappa_D\}$.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{Media/arc_view.png}
%     \label{fig:arc_view}
%     \caption{Arc view of $s$.}
% \end{figure}

%We apply the concept shown in in Fig.~\ref{fig:kappa_calc} by establishing a plane passing through points $A\bar{S}S$ called $\mathcal{A}$ and define a point $\bar{\bar{A}}$ on $\mathcal{B}$ so that $\bar{\bar{A}}A$ and $\bar{\bar{A}}S$ are colinear. It can be seen then that the distance between $\bar{\bar{A}}\bar{S}$ and $\bar{\bar{A}}S$ is equal and we define it as $r_A = \frac{1}{\kappa_A}$. We then bisect the triangle $\bar{\bar{A}}\bar{S}S$ with a line from $\bar{\bar{A}}$ to a point $S_A$ on $\bar{S}S$ such that $\bar{\bar{A}}S_A \perp \bar{S}S$. Using the similarity of triangles $ASS''$ and $\bar{\bar{A}}SS_A$ and~\eqref{eq:hs} the curvature for linkage $A$ is shown to be
\begin{comment}
    

    \kappa_A = \frac{l_C - l_A}{d ( l_A + l_C)}
\end{comment}
%and by extension
\begin{comment}
    \kappa_B &= \frac{l_D - l_B}{d ( l_B + l_D)} \\
    \kappa_C &= \frac{l_A - l_C}{d ( l_A + l_C)} = -\kappa_A \\
    \kappa_D &= \frac{l_B - l_D}{d ( l_B + l_D)} = -\kappa_B\\
\end{comment}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.45\textwidth]{Media/kappa_calc.png}
%    \caption{Plane $\mathcal{A}$ showing triangle $\bar{\bar %A}\bar{S}S$.}
%    \label{fig:kappa_calc}
%\end{figure}

Though we can calculate these lengths for each individual actuator, more significant is their  arc length subtended during it's motion. Given the dependence of the platform's pose on angles and curvatures subtended by actuators, we follow the piecewise and extensible constant curvature approach to model the position and orientation as a function of their lengths.


%It is clear that the curvature for a given actuator is dependent only on its own length \emph{and} the length of its diagonal counterpart and is likewise independent of the other two actuators. 

\subsection{Calculation of $\kappa$, $\phi$, and $s$}

To determine $\kappa$, $\phi$, and $s$ for our system, we extend the previous work on PCC models and determine the following relationships while referring to Figure~\ref{fig:configurationFull}.



\begin{equation}
\begin{aligned}
    \kappa 
          &= \frac{1}{d} \sqrt{\frac{(l_C-l_A)^2}{(l_C + l_A)^2} + \frac{(l_D-l_B)^2}{(l_D+l_B)^2}}
\end{aligned}
\end{equation}

The angle of rotation about the z-axis $\phi$ is derived as

\begin{equation}
\begin{aligned}
    \phi  
         &= tan^{-1}\left(\frac{l_Bl_C - l_Al_D}{l_Cl_D-l_Al_B}\right)
\end{aligned}
\end{equation}

% \begin{figure}[h]
%     \centering
%     \hfill
%     \begin{subfigure}[t]{0.2\textwidth}
%         \includegraphics[width=1\textwidth]{Media/coordinate_system.png}
%             \captionsetup{justification=centering}

%         \caption{Top down view of whole assembly.}    
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.2\textwidth}
%         \includegraphics[width=1\textwidth]{Media/iso_1.png}
%             \captionsetup{justification=centering}

%         \caption{Coordinate system shown on HSA platform.}
    
%     \end{subfigure}
%     \caption{Coordinate systems of HSA assembly.}
%     \label{fig:coordinate_system}
% \end{figure}


Finally the arc length $s$ is proportional to the angle $\phi$ by the curvature $\kappa$, 
\begin{equation}
    s = \frac{2}{\kappa} sin^{-1}\left(\kappa\frac{l_S}{2}\right).
\end{equation}
It is worth noting that
\begin{align*}
\lim_{\kappa\to 0} s(\kappa, l_S) &= l_S \\
\lim_{\kappa_x \to 0^{\pm}} \phi(\kappa_y, \kappa_x) &= \pm \frac{\pi}{2}\
\end{align*}
which are the cases for when the platform is in its rest position and when there is curvature only in the $YZ$ plane respectively. 

%\aman{With these values, we can then compute the transformation %$T$ from equation\ref{eq:T}from the origin to the center of the %HSA platform with its y-axis aligned normal to the platform}

%\begin{equation}
%    L = \begin{bmatrix} l_1 \\ l_2 \\ l_3 \\ l_4 \end{bmatrix}  = %\begin{bmatrix} a_{11}& a_{12}& a_{13}& a_{14} \\ a_{21}& a_{22}& %a_{23}& a_{24} \\ a_{31}& a_{32}& a_{33}& a_{34} \\ a_{41}& %a_{42}& a_{43}& a_{44} \end{bmatrix} \begin{bmatrix} \theta_1 \\ %\theta_2 \\ \theta_3 \\ \theta_4 \end{bmatrix} + \begin{bmatrix} %b_1 \\ b_2 \\ b_3 \\ b_4 \end{bmatrix}
%\end{equation}

\subsection{Calculation of position and orientation}

With the center of the top platform represented in arc parameters ($s,\kappa , \phi$), we use a D-H formulation for transformation to X ,Y, Z coordinates of the center of the top platform. We approach the forward kinematics from the base as a virtual revolute-revolute-prismatic (RRP) transformation as previously stated in \cite{Jones2010-doi:10.1177/0278364910368147}. This approach defines our transformation matrix shown in \eqref{eq:T}.
\begin{equation}
    T = \begin{bmatrix} \cos\phi\cos\kappa s & -\sin\phi & \cos\phi\sin\kappa s & \frac{\cos\phi(1-\cos\kappa s)}{\kappa} \\ \sin\phi\cos\kappa s & \cos\phi & \sin\phi\sin\kappa s & \frac{\sin\phi(1-\cos\kappa s)}{\kappa} \\ -\sin\kappa s & 0 & \cos\kappa s & \frac{\sin \kappa s}{\kappa} \\ 0 & 0 & 0 & 1 \end{bmatrix}
    \label{eq:T}
\end{equation}
The base coordinates of the system are defined in our system as - 
\begin{equation}
   B = [0 ; 0 ; 0; 1] 
   \label{eq:basezero}
\end{equation}

The position coordinates of the center point of the top platform would then be given by:
\begin{equation}
P = \begin{bmatrix}
x \\
y \\
z \\
1
\end{bmatrix}
= T\ast B
\label{eq:Pcoordinate}
\end{equation}

Further, the orientation is defined by two angles:

\begin{equation}
  \begin{bmatrix}
\alpha \\
\phi \\

\end{bmatrix}
= \begin{bmatrix}
s\kappa \\
tan^{-1}(\frac{l_Bl_C - l_Al_D}{l_Cl_D-l_Al_B}) \\

\end{bmatrix}
\label{eq:orientationvalue}
\end{equation}


\begin{figure*}[thbp]
    \centering
    \includegraphics[width= 17cm]{sequence.pdf}

    \caption{Sequence of operations with the platform for experimental validation where each frame represents the state of the platform at time = t seconds.}
    \label{fig:sequence}
\end{figure*}


==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/3Methods.tex <==
\section{Experimental Setup}
Calibration is required to map between PWM values in Pololu's software to angular displacement on each individual servo for precise and accurate control. This was done by attaching an approximately 10in rod to the end of each servo and rotating 90 degrees to determine a conversion between PWM values and servo's angle of rotation.An OptiTrack system made from four Flex 13 cameras was used to track changes in the 2x2 HSA platform. The four cameras were located in top corners of a 1 cubic meter test volume and pointed at the platform. Two rigid bodies were defined representing the dynamic top platform and the static bottom platform. 3D position and quaternion data were saved for each rigid body. We gathered all permutations on the HSAs from 0$^{\circ}$ to 180$^{\circ}$ in 30$^{\circ}$ increments. This resulted in 2401 unique states. These states were used to determine the coupling matrix ${\beta_0}$ and vector ${\beta_1}$. 

For validation , we performed a composite rotation of the platform as shown in Fig~\ref{fig:sequence}.This ensured that all the possible positions - extension, compression, bending \& rotation were combined within one single sweep. We performed this sweep for the full range of speeds the servos could generate (between 0.15 RPM and 30 RPM) 




==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/3NeuralNet.tex <==
\section{Neural Network Model}
% .5-1 pages

A single layer, feed forward network was created in MATLAB for non-linear regression as a point of comparison against the derived ECC model. The inputs to the network were the four $\theta$ variables used to actuate the HSAs and the outputs were the position of the platform's center $\bm x$ in $x, y, z$ and the imaginary parts $q_x, q_y, q_z$ of the platform's quaternion $\bm q$. The real part of the quaternion $q_w$ was not part of the output because the quaternion $\bm q$ is unit length and thus only three parts are needed to determine the fourth. The network was trained using mean square error (MSE) as the cost function and the Levenberg-Marquardt backpropagation algorithm. The 2401 theta state samples were randomly divided into training and validation sets at a 7:3 ratio. Training time for all networks were less than 1 minute on a machine with an Intel\textsuperscript{\textregistered} Core\textsuperscript{\texttrademark} i-7 and 32 GB of RAM.

Fig.~\ref{fig:NN_performance} shows the MSE plot for a network with a single hidden layer with 20 neurons and a table showing final performance of networks with various hidden layer sizes. The MSE in this training is the raw error associated with position and quaternion values. Table~\ref{tab:NN_compare} shows that the error on the validation dataset does continue to decrease with increased hidden layer size; however, this also results in an overfitting of the data, where the training error continues to decrease while the validation performance only improves marginally. The network with 20 neurons was used as the final comparison point with the ECC model because it was heuristically determined to have the best performance overall in terms of validation and test error although it should be noted that the network with only 5 neurons also performed nearly as well in terms of absolute error. 

\begin{figure}[h]
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.8\linewidth]{Media/mse_epoch_20neurons.png}    
        \label{fig:NN_mse}
        % \caption{\todo{CAPTION}}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Single layer 20 neuron training performance over time.}
    \label{fig:NN_performance}
    \vspace{-4mm}
\end{figure}

\begin{table}
    \centering
    \begin{tabularx}{.9\linewidth}{| X | X | X | X |}
        \hline
        No. \newline Neurons & No. Free Parameters & Training MSE & Validation MSE \\
        \hline
        5           & 61                           & 4.38E-5      & 4.47E-5       \\
        20          & 226                           & 7.35E-6      & 8.95E-6       \\
        50          & 556                          & 4.37E-6      & 5.77E-6       \\
        100         & 1106                           & 3.86E-6      & 6.28E-6       \\ 
        \hline
    \end{tabularx}
    \caption{Comparison of different network sizes.}
    \label{tab:NN_compare}
\end{table}


==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/4Results.tex <==
\section{Results and Discussion}
% 1 pages
% \todo{
%     \begin{itemize}
%         \item Fit of EPCC Beta matrix and $R^2$ value (plus others if applicable) 
%         \item talk about potential issues with the FPU batch we used
%     \end{itemize}
% }
  
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Media/uncoupled_length_error.png}
%     \captionsetup{justification=centering}
%     \caption{Histogram comparing error in length in the uncoupled linear estimation model.}
%     \label{fig:HSA Platform}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Media/coupled_length_error.png}
%     \captionsetup{justification=centering}
%     \caption{Stacked histogram comparing error in lengths in the coupled linear estimation model.}
%     \label{fig:HSA Platform}
% \end{figure}

\subsection{Mapping $\theta$ to length}
The basis of our model is the mapping between inputs $\vec{\theta}$ and lengths. In section~\ref{sec:HSADesign} we found the linear relationship between $\theta$ and the length $l$ of an HSA at which there is no more extensional force. As a first approximation, we use these results in an uncoupled linear model for estimating lengths of the actuators and observe significant errors against measured lengths from OptiTrack. The analysis for it is shown in Fig.~\ref{fig:coupled_errorl}A where the average error in length estimation is 4.78mm with a standard deviation of 4.7mm and a range of -9 to 16mm. This was not unexpected as the above model considers the actuators as independent structures but the 2x2 HSA platform acts as a common linkage between the four actuators producing a coupled model with interconnected links. This leads the naive model to over estimate the length of the segments and produces a wide range of errors. 

\begin{figure}
    \centering
    \includegraphics{Coupled.pdf}
    \captionsetup{justification=centering}
    \caption{(a) Error between the estimated and observed actuator length when using uncoupled mapping ; (b) Error between estimated and observed actuator length when using coupled mapping }
    \label{fig:coupled_errorl}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{boxplot.pdf}
    \captionsetup{justification=centering}
    \caption{Position error with change in velocity }
    \label{fig:position_error}
\end{figure}

By contrast when we integrate the two observations in our Coupled Length Estimation Model, as explained in the modeling section, we correct the bias and reduce the range and variance of the errors as seen in Figure~\ref{fig:coupled_errorl}. The resulting error in actuator length prediction reduces to a mean of 0.25mm with a standard deviation of 1.6mm with a range of -4 to 6 mm. Since the errors in length propagate through the model we must examine the effects on predicting position and state through the trajectory.

In Figure~\ref{fig:comparison}A we see the inputs to the sequence sequence seen in Fig~\ref{fig:sequence}. The lengths of the actuators predicted and measured are seen in Figure~\ref{fig:comparison}C.  As we can see, when the actuator is moving, we see the most agreement between the model and measurement. The greatest disagreement occurs when an actuator is meant to be held still. This is likely a result of an relationship not captured in the beta matrix. We suspect that the driving actuators, acting as a force generator are compressing the held actuators, which then are pulled or pushed. An alternative explanation where the limits of extension are the source of errors is less likely to be true since L2 and L1 have large errors at their rest state. 




%We compare the training and test results to determine the average error in distance between the measured and estimated lengths of each actuator in Fig.~\ref{fig:coupled_length_error}. We observe a significant improvement from the Uncoupled linear length estimation Model. The $R^2$ of the linear regression for the validation set was 0.958 with a mean error of 1.36 mm highlighting the closeness of the fit for our model.

% \begin{figure}[thbp]
%     \centering
%     \begin{subfigure}[t]{0.49\linewidth}
%         \includegraphics[width=0.99\linewidth]{Media/uncoupled_length_error.png}
%         \captionsetup{justification=centering}
%         \caption{Error in length in the uncoupled linear estimation model.}
%         \label{fig:uncoupled_length_error}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.49\linewidth}
%         \includegraphics[width=0.99\linewidth]{Media/coupled_length_error.png}
%         \captionsetup{justification=centering}
%         \caption{Stacked error histogram of length in the coupled linear estimation model.}
%         \label{fig:coupled_length_error}
%     \end{subfigure}
%     \caption{Histograms showing error reduction from na\"ive uncoupled to linear regression coupled estimation of actuator length as a function of $\theta$.\todo{redo as non-magnitude length errors}}
%     \label{fig:length_error}
% \end{figure}

\subsection{Piecewise Constant Curvature Model}
Figure~\ref{fig:comparison}B and D show the error propagation through the model. We cannot observe the full state of the PCC section model, but we can observe the value of $\phi$ from the Optitrack data since its merely the angle between the plane that contains the center point and the Z axis, with the XZ plane. In Figure~\ref{fig:comparison}D we see that $\phi$ is accurately captured by the model. The error of $\phi$ is between -3.4$^{\circ}$ and 3.7$^{\circ}$ with an average of -1.5$^{\circ}$. 

We can also observe $\alpha$, the angle subtended by the arc section which is a combined metric of $\kappa$ and $s$. $\alpha$ and $\phi$ encode the orientation of the platform.
We observe that $\kappa$ is well predicted from the kinematic model with a range of error between -5.85$^{\circ}$ and 0.2$^{\circ}$ and an average error of -2.8$^{\circ}$.
Therefore the model can reasonably capture the orientation of the platform. 

We compare the Cartesian coordinate of the center point with the one predicted from the model in Figure~\ref{fig:comparison}B. The result is a model which can predict the position with minimal error. When we repeat the motion at various speeds as seen in Figure ~\ref{fig:position_error} we see that for these motors, the model does not have an appreciable change in error. The figure shows the distribution of errors in the distance between the center of the platform observed and predicted. As the speed varies the mean error goes from a minimum of 5.5mm to a maximum of 5.7mm with no meaningful correlation with speed. Therefore we can conclude that for these motors and mass, the inertial effects can be ignored and a kinematic model such as ours is sufficient. 



% The analysis demonstrates the strengths of our proposed model as  able to closely estimate the measured values obtained from OptiTrack. The errors are most likely caused by material hysteresis and variability in the geometric arcs at higher rotation angles. 

% For an actuator assembly for height 123 mm and extensible length of 31mm at $180^\circ$, the low average positional error indicates advantages of this kinematic modelling in applications in orienting structures which need high extensibility. A key observation from our results is noted in Table~\ref{tab:ECC180_results}. Without 180$^\circ$ values from our data we reduce the positional error by more than 25\%. This is explained by the material behaviour of the actuators. During the continuous loading process the cell size of the HSA expands leading to lower structural rigidity and becoming prone to lateral shifts.This drawback could be rectified by modifying the size of the HSA which would ensure higher structural rigidity for higher rotation angles.   


% The estimated lengths of the actuators along the test sequence (seen in Fig~\ref{fig:sequence}) are feed to the PCC Kinematic Model. The error in the 

% which maps every actuator state to a computed $s,\kappa,\phi$ for the center $S$ of the top platform. These values are then fed to the D-H transformation, equation~\eqref{eq:T}, to determine the coordinates of the center of the top platform. When compared with the measured coordinates from OptiTrack data we see an $R^2$ value of 0.959. We also compared the orientation ($\alpha$) as a difference between estimated and measured normal of the center. Further analysis is presented in Table~\ref{tab:ECC_results}.



% \begin{figure*}[!th]
%     \centering
%     \includegraphics[width= 17cm]{Comparison.eps}
%     \captionsetup{justification=centering}
%     \caption{(a) shows the variation of servo motor angle with time ; (b) shows comparison of Observed vs Estimated position of the center of the top platform; (c) shows a comparison of Observed vs Estimated lengths of the actuators; (d) shows a comparison of Observed vs Estimated ${\phi}$ of the platform. }
%     \label{fig:comparison}
% \end{figure*}

\begin{figure*}[!th]
    \centering
    \includegraphics[width= 17cm]{Comparison.pdf}
    \captionsetup{justification=centering}
    \caption{(a) Shows the variation of servo motor angle(input) with time ; (b) Shows comparison of Observed vs Estimated position of the center of the top platform ; (c) Shows a comparison of Observed vs Estimated lengths of the actuators ; (d) Shows a comparison of Observed vs Estimated orientation angles of the platform. }
    \label{fig:comparison}
\end{figure*}




% Figures for theta, xyz, length, angles


%\begin{figure}
%    \centering
%    \includegraphics[]{xyz.eps}
%    \caption{Comparison of Measured and Estimated Coordinates}
%    \label{fig:xyz_compare}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{lengths.eps}
%    
%    \caption{Comparison of Measured and Estimated Length of all actuators}
%    \label{fig:length_compare}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{angles.eps}
%    \caption{Comparison of Measured and Estimated $\phi$}
%    \label{fig:angle_compare}
%\end{figure}



%\begin{table}[]
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%                   & \multicolumn{2}{c|}{\textbf{Positional Error (mm)}} & \multicolumn{2}{c|}{\textbf{Angular Error (deg)}} \\ \hline
%                   & \textbf{Fitting}         & %\textbf{Testing}        & \textbf{Fitting}        & %\textbf{Testing}       \\ \hline
%Average            & 4.1                       & 3.88    %                & 2.58                     & 2.79        %           \\ \hline
%Standard Deviation & 2.6                       & 2.1     %                & 1.54                     & 2.04        %           \\ \hline
%Maximum            & 13.11                     & 10.1     %               & 7.43                     & 9.1           %         \\ \hline
%Minimum            & 0.17                      & 0.15     %               & 0                        & 0.004         %         \\ \hline
%\end{tabular}
%\captionsetup{justification=centering}
%\caption{Positional and Angular error analysis for ECC %kinematic model }
%    \label{tab:ECC_results}
%    \vspace{-4mm}
%\end{table}

% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%                   & \multicolumn{2}{c|}{\textbf{Positional Error (mm)}} & \multicolumn{2}{c|}{\textbf{Angular Error (deg)}} \\ \hline
%                   & \textbf{Fitting}         & \textbf{Testing}        & \textbf{Fitting}        & \textbf{Testing}       \\ \hline
% Average            & 1.06                     & 1.13                    & 0.48                     & 0.51                   \\ \hline
% Standard Deviation & 0.53                     & 0.60                    & 0.31                     & 0.35                   \\ \hline
% Maximum            & 4.43                     & 5.20                    & 3.73                     & 2.87                    \\ \hline
% Minimum            & 0.11                     & 0.11                    & 0.02                     & 0.02                  \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Positional and Angular error analysis for Neural Network model }
%     \label{tab:NN_results}
% \end{table}


% \centering
% \begin{comment}{|c|c|c|}
% \hline
%  &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Positional Error\\ w/o 180 Deg (mm)\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Angular Error \\ w/o 180 Deg (deg)\end{tabular}} \\ \hline
%                                                               & \textbf{Testing} & \textbf{Testing} \\ \hline
% Average                                                       & 2.84             & 2.5              \\ \hline
% \begin{tabular}[c]{@{}c@{}}Standard\\  Deviation\end{tabular} & 1.49             & 1.69             \\ \hline
% Maximum                                                       & 7.08             & 6.89             \\ \hline
% Minimum                                                       & 0.15             & 0.0051           \\ \hline

% \captionsetup{justification=centering}
% \caption{Positional and Angular error analysis for ECC kinematic model without 180$^\circ$ }
%     \label{tab:ECC180_results}
% \end{comment}

% \begin{comment}
%     \centering
%     % \hfill
%     \begin{subfigure}[t]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Media/position_error_ecc.png}
%         % \caption{}
%         \label{fig:position_error_NN}
%     \end{subfigure}
%     % \hfill
%     % \vskip\baselineskip
%     % \vfill
%     \begin{subfigure}[t]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Media/angular_error_ecc.png}
%         % \caption{}
%         \label{fig:angular_error_NN}
%     \end{subfigure}
%     % \hfill
%     \captionsetup{justification=centering}

%     \caption{Stacked error histograms for distance and angle}
%     \label{fig:model_errors}
%     \vspace{-4mm}
% \end{comment}


% \subsection{ECC and Shallow Network comparison}
% Fig.~\ref{fig:model_errors} shows histogram plots of error comparing the ECC model on the left and the neural network model on the right in both absolute position $\|\bm x' - \bm x^*\|$ and pointing direction $\psi=\angle(y',y^*)$ of the center of the platform where $a'$ and $a^*$ denote the measured and predicted values respectively.

% In both cases, position and orientation, the network outperformed the ECC model with lower means and standard deviations. While performative, the neural network does not account for the actual geometry of the assembly and so cannot be easily extended to planing. It also has no underlying insight, so extending it to dynamics would require training a separate network. By contrast the ECC model fully characterizes the assembly in space enabling planning.  Furthermore, the ECC model compresses the information coded in the $\theta$ states into only 5 free parameters between the circulant $\beta_0$ matrix and scalar $\beta_1$ while the 20 neuron network uses 626 parameters to encode the same information. In the end there is a case to be made for using a simple network in situations where only positional and angular accuracy is needed; however, ultimately the ECC model offers much more in the way of full fledged robotics control while operating on nearly the same performance level. 

% \subsection{Errors in Modeling and Data Recording}
% The leading contributor to error in this paper is the hysteresis experienced by the FPU50 HSAs. When returning to rest state, the system saw individual actuator deviations up to 2mm. This results in rest state angles varying by as much as 1.9 to 2.6 degrees. Calibration error within the OptiTrack system was present but minimized to the best extent possible. Care was taken to ensure the device was kept at a constant temperature and vibrations during recording were minimized following manufacturer recommendations \cite{optitrack_2019}. Calibration in 3D was within $\pm0.2mm$ which can result in errors as large as $0.4^\circ$.Another potential error in the system was the stability of the batch of FPU50 used for these experiments. The batch used in our testing has shown faster than normal deterioration in brittleness and impact strength. It is the opinion of the authors that this would have little effect of the data presented here but we would be remissed not to present it.
%   %compared to EPCC
%   %comparison vs neural net
%   %number of neurons vs accuracy (mean and std.)
%   %number of free parameters between models (4 parameters for EPCC vs hundreds parameters on NN?)
%   %EPCC more useful for prediction (dynamics and system understanding, performance w/ same number of parameters) with multi segment arms
%   % to discuss the importance of orientation (something we don't get with EPCC).
 
%   %tradeoff between the EPCC models and NN
  
%   %better understanding of physical happenings & multi segment
  


==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/5Conclusion.tex <==
\section{Conclusion and Future Work}

In this paper we established that Piecewise Constant Curvature models (PCC) are good forward kinematic models for a 2x2 handed shearing auxetic platform when interaction between HSAs is modeled. This is the first model of HSA platforms and shows that soft robotics modeling techniques can be adapted to HSA systems.  In comparison with a naive approach,  a model with coupling is found to be more accurate for predicting the lengths of the actuators. These can then be mapped into position and orientation of the HSA assembly's top platform. Over the range of Servo motor actuation, this model shows no degradation with increased speed.

Now that HSA platforms can be modeled they can be used more fully in robotic applications beyond gripping. Future work includes integrating our model with a controls framework for specific applications. Additionally, the platforms we have designed have only constituted a single link in the PCC framework. Extending this to a multi segment robotic arm made from HSAs is a a logical next step. 


==> Extensible PCC Model of HSA platforms (ICRA2022) Arxiv/Notes.tex <==
We should put the theta mapping after the ECC Extension

==> Notes.tex <==
We should put the theta mapping after the ECC Extension
